Generative Code Modeling with Graphs

Generative models for source code are an interesting structured prediction problem, requiring to reason about both hard syntactic and semantic constraints as well as about natural, likely programs. We present a novel model for this problem that uses a graph to represent the intermediate state of the generated output. The generative procedure interleaves grammar-driven expansion steps with graph augmentation and neural message passing steps. An experimental evaluation shows that our new model can generate semantically meaningful expressions, outperforming a range of strong baselines.

==> figures/gensteps-old.tex <==
\section{Generation Steps}
The following figure shows in detail the steps shown in \autoref{fig:NAGGraphExample}.

\begin{figure}[h]
    \centering
    \begin{minipage}[b]{.49\textwidth}
    \textbf{Initial State} \\
    \resizebox{\columnwidth}{!}{
    \begin{tikzpicture}[nag]
      \node[nontermNode] (0-10) at (0,0)
          {0
           \nodepart{two} \code{Expr}
           \nodepart{three} };

      \node[contextNode, anchor=north] (contextLastI) at ($(4.south) + (0, -.7*\vdist)$)
          { 1 \nodepart{two} \code{i} };
      \node[contextNode, anchor=north] (contextLastJ) at ($(8.south) + (0, -.7*\vdist)$)
          { 2 \nodepart{two} \code{j} };

      \draw[-, thick]
       ($(contextLastI.north west) + (-\nodehdist, .2*\vdist)$) edge[thin, dashed] ($(contextLastJ.north east) + (\nodehdist, .2*\vdist)$)
       ;
    \end{tikzpicture}%
    }%
  \end{minipage}
  \begin{minipage}[b]{.49\textwidth}
    \textbf{Step 1} \\
    \resizebox{\columnwidth}{!}{
    \begin{tikzpicture}[nag]
      \node[nontermNode] (0-10) at (0,0)
          {0
           \nodepart{two} \code{Expr}
           \nodepart{three} };
      \node[nontermNode] (3-5) at ($(0-10.south) + (-3,-\vdist)$)
          {3
           \nodepart{two} \code{Expr}
           \nodepart{three} };
      \node[termNode] (6) at ($(0-10.south) + (0,-\vdist)$)
          {
           \nodepart{two} \code{-}};
      \node[nontermNode] (7-9) at ($(0-10.south) + (3,-\vdist)$)
          {
           \nodepart{two} \code{Expr}
           \nodepart{three} };

      \gramExpThree{2}{0-10}{3-5}{6}{7-9};

      \node[contextNode, anchor=north] (contextLastI) at ($(4.south) + (0, -.7*\vdist)$)
          { 1 \nodepart{two} \code{i} };
      \node[contextNode, anchor=north] (contextLastJ) at ($(8.south) + (0, -.7*\vdist)$)
          { 2 \nodepart{two} \code{j} };

      \draw[-, thick]
       (0-10.west) edge[childEdge, bend right=15] node[above]{\tiny 1} ($(3-5.north west) + (\nodehdist,0)$)
       ($(contextLastI.north west) + (-\nodehdist, .2*\vdist)$) edge[thin, dashed] ($(contextLastJ.north east) + (\nodehdist, .2*\vdist)$)
       ;
    \end{tikzpicture}%
    }%
  \end{minipage}
  \vspace{2em}

  \begin{minipage}[b]{.49\textwidth}
    \textbf{Step 2} \\
    \resizebox{\columnwidth}{!}{
    \begin{tikzpicture}[nag]
      \node[nontermNode] (0-10) at (0,0)
          {0
           \nodepart{two} \code{Expr}
           \nodepart{three} };
      \node[nontermNode] (3-5) at ($(0-10.south) + (-3,-\vdist)$)
          {3
           \nodepart{two} \code{Expr}
           \nodepart{three} };
      \node[termNode] (4) at ($(3-5.south) + (0,-\vdist)$)
          {4
           \nodepart{two} \code{i}};
      \node[termNode] (6) at ($(0-10.south) + (0,-\vdist)$)
          {
           \nodepart{two} \code{-}};
      \node[nontermNode] (7-9) at ($(0-10.south) + (3,-\vdist)$)
          {
           \nodepart{two} \code{Expr}
           \nodepart{three} };

      \gramExpThree{2}{0-10}{3-5}{6}{7-9};
      \gramExpOne{1}{3-5}{4};

      \node[contextNode, anchor=north] (contextLastI) at ($(4.south) + (0, -.7*\vdist)$)
          { 1 \nodepart{two} \code{i} };
      \node[contextNode, anchor=north] (contextLastJ) at ($(8.south) + (0, -.7*\vdist)$)
          { 2 \nodepart{two} \code{j} };

      \draw[-, thick]
       ($(3-5.south west) + (\nodehdist,0)$) edge[childEdge]      node[right]{\tiny 2} ($(4.north west) + (\nodehdist,0)$)
       ($(contextLastI.north) + (-\nodehdist,0)$)         edge[nextUseEdge] node[right]{\tiny 2} ($(4.south) + (-\nodehdist,0)$)

       ($(contextLastI.north west) + (-\nodehdist, .2*\vdist)$) edge[thin, dashed] ($(contextLastJ.north east) + (\nodehdist, .2*\vdist)$)
       ;
    \end{tikzpicture}%
    }%
  \end{minipage}
  \begin{minipage}[b]{.49\textwidth}
    \textbf{Step 3} \\
    \resizebox{\columnwidth}{!}{
    \begin{tikzpicture}[nag]
      \node[nontermNode] (0-10) at (0,0)
          {0
           \nodepart{two} \code{Expr}
           \nodepart{three} };
      \node[nontermNode] (3-5) at ($(0-10.south) + (-3,-\vdist)$)
          {3
           \nodepart{two} \code{Expr}
           \nodepart{three} 5};
      \node[termNode] (4) at ($(3-5.south) + (0,-\vdist)$)
          {4
           \nodepart{two} \code{i}};
      \node[termNode] (6) at ($(0-10.south) + (0,-\vdist)$)
          {
           \nodepart{two} \code{-}};
      \node[nontermNode] (7-9) at ($(0-10.south) + (3,-\vdist)$)
          {
           \nodepart{two} \code{Expr}
           \nodepart{three} };

      \gramExpThree{2}{0-10}{3-5}{6}{7-9};
      \gramExpOne{1}{3-5}{4};

      \node[contextNode, anchor=north] (contextLastJ) at ($(8.south) + (0, -.7*\vdist)$)
          { 2 \nodepart{two} \code{j} };

      \draw[-, thick]

       ($(4.north)$) edge[parentEdge] node[right]{\tiny 3} ($(3-5.south east) + (-\nodehdist,0)$)

       ($(contextLastI.north west) + (-\nodehdist, .2*\vdist)$) edge[thin, dashed] ($(contextLastJ.north east) + (\nodehdist, .2*\vdist)$)
       ;
    \end{tikzpicture}%
    }%
  \end{minipage}
  \vspace{2em}

  \begin{minipage}[b]{.49\textwidth}
    \textbf{Step 4} \\
    \resizebox{\columnwidth}{!}{
    \begin{tikzpicture}[nag]
      \node[nontermNode] (0-10) at (0,0)
          {0
           \nodepart{two} \code{Expr}
           \nodepart{three} };
      \node[nontermNode] (3-5) at ($(0-10.south) + (-3,-\vdist)$)
          {3
           \nodepart{two} \code{Expr}
           \nodepart{three} 5};
      \node[termNode] (4) at ($(3-5.south) + (0,-\vdist)$)
          {4
           \nodepart{two} \code{i}};
      \node[termNode] (6) at ($(0-10.south) + (0,-\vdist)$)
          {6
           \nodepart{two} \code{-}};
      \node[nontermNode] (7-9) at ($(0-10.south) + (3,-\vdist)$)
          {
           \nodepart{two} \code{Expr}
           \nodepart{three} };

      \gramExpThree{2}{0-10}{3-5}{6}{7-9};
      \gramExpOne{1}{3-5}{4};

      \node[contextNode, anchor=north] (contextLastJ) at ($(8.south) + (0, -.7*\vdist)$)
          { 2 \nodepart{two} \code{j} };

      \draw[-, thick]
       ($(0-10.south west) + (\nodehdist,0)$) edge[childEdge]       node[right]{\tiny 4} ($(6.north west)$)
       ($(3-5.east)$)                         edge[nextSiblingEdge] node[above]{\tiny 4} ($(6.west)$)
       ($(4.north)$)                          edge[nextTokenEdge]   node[below]{\tiny 4} ($(6.south west)$)

       ($(contextLastI.north west) + (-\nodehdist, .2*\vdist)$) edge[thin, dashed] ($(contextLastJ.north east) + (\nodehdist, .2*\vdist)$)
       ;
    \end{tikzpicture}%
    }%
  \end{minipage}
  \begin{minipage}[b]{.49\textwidth}
    \textbf{Step 5} \\
    \resizebox{\columnwidth}{!}{
    \begin{tikzpicture}[nag]
      \node[nontermNode] (0-10) at (0,0)
          {0
           \nodepart{two} \code{Expr}
           \nodepart{three} };
      \node[nontermNode] (3-5) at ($(0-10.south) + (-3,-\vdist)$)
          {3
           \nodepart{two} \code{Expr}
           \nodepart{three} 5};
      \node[termNode] (4) at ($(3-5.south) + (0,-\vdist)$)
          {4
           \nodepart{two} \code{i}};
      \node[termNode] (6) at ($(0-10.south) + (0,-\vdist)$)
          {6
           \nodepart{two} \code{-}};
      \node[nontermNode] (7-9) at ($(0-10.south) + (3,-\vdist)$)
          {7
           \nodepart{two} \code{Expr}
           \nodepart{three} };

      \gramExpThree{2}{0-10}{3-5}{6}{7-9};
      \gramExpOne{1}{3-5}{4};

      \node[contextNode, anchor=north] (contextLastJ) at ($(8.south) + (0, -.7*\vdist)$)
          { 2 \nodepart{two} \code{j} };

      \draw[-, thick]
       ($(0-10.south west) + (\nodehdist,0)$) edge[childEdge, bend right=15]     node[above,xshift=2mm,yshift=-1mm]{\tiny 5} ($(7-9.north west)$)
       ($(6.south)$)                          edge[nextSiblingEdge, bend right=12] node[above]{\tiny 5} ($(7-9.west)$)

       ($(contextLastI.north west) + (-\nodehdist, .2*\vdist)$) edge[thin, dashed] ($(contextLastJ.north east) + (\nodehdist, .2*\vdist)$)
       ;
    \end{tikzpicture}%
    }%
  \end{minipage}
  \vspace{2em}

  \begin{minipage}[b]{.49\textwidth}
    \textbf{Step 6} \\
    \resizebox{\columnwidth}{!}{
    \begin{tikzpicture}[nag]
      \node[nontermNode] (0-10) at (0,0)
          {0
           \nodepart{two} \code{Expr}
           \nodepart{three} };
      \node[nontermNode] (3-5) at ($(0-10.south) + (-3,-\vdist)$)
          {3
           \nodepart{two} \code{Expr}
           \nodepart{three} 5};
      \node[termNode] (4) at ($(3-5.south) + (0,-\vdist)$)
          {4
           \nodepart{two} \code{i}};
      \node[termNode] (6) at ($(0-10.south) + (0,-\vdist)$)
          {6
           \nodepart{two} \code{-}};
      \node[nontermNode] (7-9) at ($(0-10.south) + (3,-\vdist)$)
          {7
           \nodepart{two} \code{Expr}
           \nodepart{three} };
      \node[termNode] (8) at ($(7-9.south) + (0,-\vdist)$)
          {8
           \nodepart{two} \code{j}};

      \gramExpThree{2}{0-10}{3-5}{6}{7-9};
      \gramExpOne{1}{3-5}{4};
      \gramExpOne{1}{7-9}{8};

      \node[contextNode, anchor=north] (contextLastJ) at ($(8.south) + (0, -.7*\vdist)$)
          { 2 \nodepart{two} \code{j} };

      \draw[-, thick]
       ($(7-9.south west) + (\nodehdist,0)$)  edge[childEdge]     node[right]{\tiny 6} ($(8.north west) + (\nodehdist,0)$)
       ($(6.south west) + (0.7*\nodehdist,0)$)    edge[nextTokenEdge] node[below]{\tiny 6} ($(8.west)$)
       ($(contextLastJ.north) + (-\nodehdist,0)$) edge[nextUseEdge] node[right]{\tiny 6} ($(8.south) + (-\nodehdist,0)$)

       ($(contextLastI.north west) + (-\nodehdist, .2*\vdist)$) edge[thin, dashed] ($(contextLastJ.north east) + (\nodehdist, .2*\vdist)$)
       ;
    \end{tikzpicture}%
    }%
  \end{minipage}
  \begin{minipage}[b]{.49\textwidth}
    \textbf{Step 7} \\
    \resizebox{\columnwidth}{!}{
    \begin{tikzpicture}[nag]
      \node[nontermNode] (0-10) at (0,0)
          {0
           \nodepart{two} \code{Expr}
           \nodepart{three} };
      \node[nontermNode] (3-5) at ($(0-10.south) + (-3,-\vdist)$)
          {3
           \nodepart{two} \code{Expr}
           \nodepart{three} 5};
      \node[termNode] (4) at ($(3-5.south) + (0,-\vdist)$)
          {4
           \nodepart{two} \code{i}};
      \node[termNode] (6) at ($(0-10.south) + (0,-\vdist)$)
          {6
           \nodepart{two} \code{-}};
      \node[nontermNode] (7-9) at ($(0-10.south) + (3,-\vdist)$)
          {7
           \nodepart{two} \code{Expr}
           \nodepart{three} 9};
      \node[termNode] (8) at ($(7-9.south) + (0,-\vdist)$)
          {8
           \nodepart{two} \code{j}};

      \gramExpThree{2}{0-10}{3-5}{6}{7-9};
      \gramExpOne{1}{3-5}{4};
      \gramExpOne{1}{7-9}{8};

      \draw[-, thick]
       ($(8.north west) + (\nodehdist,0)$) edge[parentEdge, bend right=24] node[right,xshift=.5mm,yshift=-.5mm]{\tiny 7} ($(7-9.south east) + (-\nodehdist,0)$)

       ($(contextLastI.north west) + (-\nodehdist, .2*\vdist)$) edge[thin, dashed] ($(contextLastJ.north east) + (\nodehdist, .2*\vdist)$)
       ;
    \end{tikzpicture}%
    }\vspace{1.5em}%
  \end{minipage}
  \vspace{2em}

  \begin{minipage}[b]{.49\textwidth}
    \textbf{Step 8} \\
    \resizebox{\columnwidth}{!}{
    \begin{tikzpicture}[nag]
      \node[nontermNode] (0-10) at (0,0)
          {0
           \nodepart{two} \code{Expr}
           \nodepart{three} 10};
      \node[nontermNode] (3-5) at ($(0-10.south) + (-3,-\vdist)$)
          {3
           \nodepart{two} \code{Expr}
           \nodepart{three} 5};
      \node[termNode] (4) at ($(3-5.south) + (0,-\vdist)$)
          {4
           \nodepart{two} \code{i}};
      \node[termNode] (6) at ($(0-10.south) + (0,-\vdist)$)
          {6
           \nodepart{two} \code{-}};
      \node[nontermNode] (7-9) at ($(0-10.south) + (3,-\vdist)$)
          {7
           \nodepart{two} \code{Expr}
           \nodepart{three} 9};
      \node[termNode] (8) at ($(7-9.south) + (0,-\vdist)$)
          {8
           \nodepart{two} \code{j}};

      \gramExpThree{2}{0-10}{3-5}{6}{7-9};
      \gramExpOne{1}{3-5}{4};
      \gramExpOne{1}{7-9}{8};

      \draw[-, thick]
       ($(3-5.north east) + (-\nodehdist,0)$)  edge[parentEdge, bend left=31]  node[above]{\tiny 8} ($(0-10.north east) + (-1.7*\nodehdist,0)$)
       ($(6.north)$)                           edge[parentEdge, bend right=15] node[above,xshift=.5mm,yshift=-.5mm]{\tiny 8} ($(0-10.south east) + (-\nodehdist,0)$)
       ($(7-9.north east) + (-\nodehdist,0)$) edge[parentEdge, bend right=5]  node[above]{\tiny 8} ($(0-10.east)$)

       ($(contextLastI.north west) + (-\nodehdist, .2*\vdist)$) edge[thin, dashed] ($(contextLastJ.north east) + (\nodehdist, .2*\vdist)$)
       ;
    \end{tikzpicture}%
    }%
  \end{minipage}
\end{figure}


==> figures/graph-old.tex <==
\newcommand{\vdist}{0.725}
\newcommand{\nodehdist}{0.3}
\begin{figure}[H]
  \resizebox{\columnwidth}{!}{
  \begin{tikzpicture}[nag]
    \node[nontermNode] (0-10) at (0,0)
        {0
         \nodepart{two} \code{Expr}
         \nodepart{three} 10};
    \node[nontermNode] (3-5) at ($(0-10.south) + (-3,-\vdist)$)
        {3
         \nodepart{two} \code{Expr}
         \nodepart{three} 5};
    \node[termNode] (4) at ($(3-5.south) + (0,-\vdist)$)
        {4
         \nodepart{two} \code{i}};
    \node[termNode] (6) at ($(0-10.south) + (0,-\vdist)$)
        {6
         \nodepart{two} \code{-}};
    \node[nontermNode] (7-9) at ($(0-10.south) + (3,-\vdist)$)
        {7
         \nodepart{two} \code{Expr}
         \nodepart{three} 9};
    \node[termNode] (8) at ($(7-9.south) + (0,-\vdist)$)
        {8
         \nodepart{two} \code{j}};

    \gramExpThree{2}{0-10}{3-5}{6}{7-9};
    \gramExpOne{1}{3-5}{4};
    \gramExpOne{1}{7-9}{8};

%    \node[contextNode, anchor=south east] (contextLastTok) at ($(5.north west) + (-1, 0.7)$)
%        { \code{=} \nodepart{two} 1 };
    \node[contextNode, anchor=north] (contextLastI) at ($(4.south) + (0, -.7*\vdist)$)
        { 1 \nodepart{two} \code{i} };
    \node[contextNode, anchor=north] (contextLastJ) at ($(8.south) + (0, -.7*\vdist)$)
        { 2 \nodepart{two} \code{j} };

    \draw[-, thick]
     (0-10.west) edge[childEdge, bend right=15] node[above]{\tiny 1} ($(3-5.north west) + (\nodehdist,0)$)

     ($(3-5.south west) + (\nodehdist,0)$) edge[childEdge]      node[right]{\tiny 2} ($(4.north west) + (\nodehdist,0)$)
%     ($(contextLastTok.south east)$)             edge[nextTokenEdge]  node[above]{\tiny 2} ($(5.north west)$)
     ($(contextLastI.north) + (-\nodehdist,0)$)         edge[nextUseEdge] node[right]{\tiny 2} ($(4.south) + (-\nodehdist,0)$)

     ($(4.north)$) edge[parentEdge] node[right]{\tiny 3} ($(3-5.south east) + (-\nodehdist,0)$)

     ($(0-10.south west) + (\nodehdist,0)$) edge[childEdge]       node[right]{\tiny 4} ($(6.north west)$)
     ($(3-5.east)$)                         edge[nextSiblingEdge] node[above]{\tiny 4} ($(6.west)$)
     ($(4.north)$)                          edge[nextTokenEdge]   node[below]{\tiny 4} ($(6.south west)$)

     ($(0-10.south west) + (\nodehdist,0)$) edge[childEdge, bend right=15]     node[above,xshift=2mm,yshift=-1mm]{\tiny 5} ($(7-9.north west)$)
     ($(6.south)$)                          edge[nextSiblingEdge, bend right=12] node[above]{\tiny 5} ($(7-9.west)$)

     ($(7-9.south west) + (\nodehdist,0)$)  edge[childEdge]     node[right]{\tiny 6} ($(8.north west) + (\nodehdist,0)$)
     ($(6.south west) + (0.7*\nodehdist,0)$)    edge[nextTokenEdge] node[below]{\tiny 6} ($(8.west)$)
     ($(contextLastJ.north) + (-\nodehdist,0)$) edge[nextUseEdge] node[right]{\tiny 6} ($(8.south) + (-\nodehdist,0)$)

     ($(8.north west) + (\nodehdist,0)$) edge[parentEdge, bend right=24] node[right,xshift=.5mm,yshift=-.5mm]{\tiny 7} ($(7-9.south east) + (-\nodehdist,0)$)

     ($(3-5.north east) + (-\nodehdist,0)$)  edge[parentEdge, bend left=31]  node[above]{\tiny 8} ($(0-10.north east) + (-1.7*\nodehdist,0)$)
     ($(6.north)$)                           edge[parentEdge, bend right=15] node[above,xshift=.5mm,yshift=-.5mm]{\tiny 8} ($(0-10.south east) + (-\nodehdist,0)$)
     ($(7-9.north east) + (-\nodehdist,0)$) edge[parentEdge, bend right=5]  node[above]{\tiny 8} ($(0-10.east)$)

     ($(contextLastI.north west) + (-\nodehdist, .2*\vdist)$) edge[thin, dashed] ($(contextLastJ.north east) + (\nodehdist, .2*\vdist)$)
     ;
  \end{tikzpicture}%
  }%
  \vspace*{-1.5mm}%
  \caption{\label{fig:NAGGraphExample}Example AST with attribute dependencies.
    Each AST node (labeled by a terminal or non-terminal) has either one or two
    associated attribute nodes, shown to the left/right of the label.
    Edge style/color indicates edge type and edge labels indicate the order in
    which edges are used.}
  \end{figure}


==> text/nagdetails.tex <==


To define our model precisely, we give pseudo-code for our decoding procedure,
which draws edges as needed.
To generate training data, we can run the same procedure, substituting ground
truth for sampled values.

For an AST node $v$, we use \inhNode{v} (resp.\ \synNode{v}) to refer to its
inherited (resp.\ synthesized) attribute node.
We associate a \emph{node state} \nodeState{v} with each node $v$, \ie,
$\nodeState{\synNode{v}}$ refers to the state of the synthesized attribute of
node $v$.
Similarly, we use \nodeLabel{v} to refer to node label of node $v$.

Our full decoding procedure is shown in \rA{alg:decoder}.
To generate code for a context $c$ and variables $v_1, \ldots, v_k$, we first
encode $c$ into some vector $\nodeState{c}$ and create a fresh root node $r$,
setting $\nodeState{r} = \nodeState{c}$.
We then call the procedure \textsf{Expand} shown in \rA{alg:decoder}.

\renewcommand{\algorithmicrequire}{\textbf{Input:}}
\begin{algorithm}
  \begin{algorithmic}[1]
    \Require Node $v$ to expand, $\mathcal{V}$ set of variables
      \Comment{We expect $\nodeState{\inhNode{v}}$ to be defined on call.}
    \State{$\mathit{rhs} \leftarrow \mathsf{pickProduction}(\ell_v, \nodeState{\inhNode{v}})$}
      \Comment{Pick production rule for nonterminal kind $\ell_v$ (\cf \rEq{eq:pickProduction}).}
    \State{$\mathit{lastSib} \leftarrow \bot$}
    \State{$\mathcal{E}_\uparrow \leftarrow \emptyset$}
    \For{$\mathit{nodeKind}\ \text{in}\ \mathit{rhs}$}
      \State{$v', \inhNode{v'}, \synNode{v'} \leftarrow \mathsf{newChildOfKind}(v, \mathit{nodeKind})$}
        \Comment{Create fresh node ids and note production.}
      \State{$\mathcal{E}_\downarrow \leftarrow \{ (\inhNode{v}, \text{Child}) \}$}
      \If{$\mathit{lastSib} \neq \bot$}\Comment{Add connection from sibling, if it exists.}
        \State{$\mathcal{E}_\downarrow \leftarrow \mathcal{E}_\downarrow \cup
          \{ (\synNode{\mathit{lastSib}}, \text{Parent}) \}$}
      \EndIf
      \State{$\mathit{lastSib} \leftarrow v'$}
      \If{$\mathit{nodeKind}$ has no known productions}
        \State{$\mathcal{E}_\downarrow \leftarrow \mathcal{E}_\downarrow \cup
          \{ (\synNode{\mathit{lastToken}}, \text{NextToken}) \}$}
          \Comment{Add edge from last token.}
        \State{$\mathit{lastToken} \leftarrow v'$}
        \If{$\mathit{nodeKind} = \text{Variable}$}
          \State{$\nodeLabel{v'} \leftarrow \mathsf{pickVariable}(\mathcal{V},
            \nodeState{\inhNode{v}})$}          
          \Comment{Pick from variables in scope (\cf \rEq{eq:pickVariable}).}
          \State{$\mathcal{E}_\downarrow \leftarrow \mathcal{E}_\downarrow \cup
            \{ (\synNode{\mathcal{V}(\nodeLabel{v'})}, \text{NextUse}) \}$}
          \Comment{Add edge from last use of variable.}
          \State{$\mathcal{V}(\nodeLabel{v'}) \leftarrow v'$}
        \Else
          \State{$\nodeLabel{v'} \leftarrow \mathit{nodeKind}$}
        \EndIf
      \EndIf
      \State{$\nodeState{\inhNode{v'}} \leftarrow \mathsf{edgePropagate}(\nodeLabel{v'}, \mathcal{E}_\downarrow)$}
        \Comment{Compute inherited neural attributes for $v'$ (\cf \rEq{eq:edgePropagate}).}
      \If{$\mathit{nodeKind}$ has productions}
        \State{$\mathsf{Expand}(v')$} \Comment{Recursively expand nonterminals.}
      \Else
        \State{$\nodeState{\synNode{v'}} \leftarrow \nodeState{\inhNode{v'}}$}
      \EndIf
      \State{$\mathcal{E}_\uparrow \leftarrow \mathcal{E}_\uparrow \cup \{ (\synNode{v'}, \text{Parent}) \}$}
    \EndFor
    \State{$\nodeState{\synNode{v}} \leftarrow \mathsf{edgePropagate}(\nodeLabel{v}, \mathcal{E}_\uparrow)$}
    \Comment{Compute synthesised neural attributes for $v'$ (\cf \rEq{eq:edgePropagate}).}
  \end{algorithmic}
  \caption{\ourmodel decoding procedure ``\textsf{Expand}''.}
  \label{alg:decoder}
\end{algorithm}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "exprSynth"
%%% End:

